SDD-4DGS: Static-Dynamic Aware Decoupling in Gaussian Splatting for 4D Scene Reconstruction

Dynamic and static components in scenes often exhibit distinct properties, yet most 4D reconstruction methods treat them indiscriminately, leading to suboptimal performance in both cases. This work introduces SDD-4DGS, the first framework for static-dynamic decoupled 4D scene reconstruction based on Gaussian Splatting. Our approach is built upon a novel probabilistic dynamic perception coefficient that is naturally integrated into the Gaussian reconstruction pipeline, enabling adaptive separation of static and dynamic components. With carefully designed implementation strategies to realize this theoretical framework, our method effectively facilitates explicit learning of motion patterns for dynamic elements while maintaining geometric stability for static structures. Extensive experiments on five benchmark datasets demonstrate that SDD-4DGS consistently outperforms state-of-the-art methods in reconstruction fidelity, with enhanced detail restoration for static structures and precise modeling of dynamic motions. The code will be released.

==> tabs/miccai2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\label{tab:my-table}
\centering
\begin{tabular}{llllllllll}
\Xhline{2pt}
\multicolumn{1}{c}{}                                                                                     & \multicolumn{3}{c}{\textbf{Pulling}}                                                                                    & \multicolumn{3}{c}{\textbf{Cutting}}                                                                                                            & \multicolumn{3}{c}{\textbf{Ave}}                                                                                        \\
\multicolumn{1}{c}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Ours \\ Benchmark\end{tabular}}}} & \multicolumn{1}{c}{PSNR  $\uparrow$} & \multicolumn{1}{c}{SSIM $\uparrow$} & \multicolumn{1}{c}{LPIPS $\downarrow$} & \multicolumn{1}{c}{PSNR  $\uparrow$} & \multicolumn{1}{c}{SSIM $\uparrow$} & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}LPIPS $\downarrow$} & \multicolumn{1}{c}{PSNR  $\uparrow$} & \multicolumn{1}{c}{SSIM $\uparrow$} & \multicolumn{1}{c}{LPIPS $\downarrow$} \\ \hline
SurgicalGS                                                                                               & 27.87                                    & 0.926                               & 0.091                                  & 34.70                                    & 0.951                               & 0.086                                                          & {\color[HTML]{000000} 31.28}             & {\color[HTML]{000000} 0.938}        & {\color[HTML]{000000} 0.088}           \\
EndoGS                                                                                                   & 25.18                                    & 0.901                               & 0.128                                  & 33.50                                    & 0.95                                & 0.106                                                          & 29.34                                    & 0.925                               & 0.117                                  \\
LenPlane                                                                                                 & 24.10                                    & 0.846                               & 0.177                                  & 29.43                                    & 0.907                               & 0.165                                                          & 26.76                                    & 0.876                               & 0.171                                  \\
\rowcolor[HTML]{EFEFEF} 
ImLight(Ours)                                                                                            & \textbf{28.28}                           & \textbf{0.930}                      & \textbf{0.083}                         & \textbf{35.44}                           & \textbf{0.954}                      & \textbf{0.078}                                                 & \textbf{31.86}                           & \textbf{0.942}                      & \textbf{0.080}                         \\ \Xhline{2pt}
\end{tabular}
\caption{Quantitative evaluation under extensive camera movement and moving point light source conditions. Our ImLight method maintains superior performance across both surgical scenarios.}

\end{table*}

==> tabs/miccal.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\begin{tabular}{lccccccccc}
\Xhline{2pt}
                                         & \multicolumn{3}{c}{\textbf{Pulling}}                        & \multicolumn{3}{c}{\textbf{Cutting}}                                                & \multicolumn{3}{c}{\textbf{Ave}}                                                           \\
\multirow{-2}{*}{\textbf{EndoNerf}} & PSNR  $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR  $\uparrow$ & SSIM $\uparrow$ & \cellcolor[HTML]{EFEFEF}LPIPS $\downarrow$ & PSNR  $\uparrow$         & SSIM $\uparrow$              & LPIPS $\downarrow$           \\ \hline
SurgicalGS                               & 38.11                & 0.963           & 0.04               & 37.03                & 0.960           & 0.033                                      & {\color[HTML]{000000} 37.57} & {\color[HTML]{000000} 0.961} & {\color[HTML]{000000} 0.038} \\
EndoGS                                   & 37.03                & 0.956           & 0.09               & 37.86                & 0.969           & 0.03                                       & 37.44                        & 0.962                        & 0.061                        \\
LenPlane                                 & 36.28                & 0.936           & 0.08               & 35.71                & 0.933           & 0.067                                      & 35.99                        & 0.934                        & 0.076                        \\
EndoSurf                                 & 36.41                & 0.96            & 0.11               & 36.41                & 0.960           & 0.114                                      & 36.41                        & 0.960                        & 0.114                        \\
\rowcolor[HTML]{EFEFEF} 
ImLight(Ours)                            & \textbf{38.53}       & \textbf{0.966}  & \textbf{0.04}      & \textbf{37.61}       & \textbf{0.963}  & \textbf{0.03}                              & \textbf{38.07}               & \textbf{0.964}               & \textbf{0.035}               \\ \Xhline{2pt}
\end{tabular}
\caption{Quantitative evaluation of novel view synthesis on the EndoNeRF dataset with two surgical scenarios. Our ImLight method achieves the best performance across all metrics, with a notable average PSNR improvement of 0.5dB over the second-best method.}\label{tab:my-table}
\end{table*}
